Correcting Negative Bias in Large Language Models through Negative Attention Score Alignment

A binary decision task, like yes-no questions or answer verification, reflects a significant real-world scenario such as where users look for confirmation about the correctness of their decisions on specific issues. In this work, we observe that language models exhibit a negative bias in the binary decisions of complex reasoning tasks. Based on our observations and the rationale about attention-based model dynamics, we propose a negative attention score (NAS) to systematically and quantitatively formulate negative bias. Based on NAS, we identify attention heads that attend to negative tokens provided in the instructions as answer candidate of binary decisions, regardless of the question in the prompt, and validate their association with the negative bias. Additionally, we propose the negative attention score alignment (NASA) method, which is a parameter-efficient fine-tuning technique to address the extracted negatively biased attention heads. Experimental results from various domains of reasoning tasks and large model search space demonstrate that NASA significantly reduces the gap between precision and recall caused by negative bias while preserving their generalization abilities.

==> algorithms/head_detection.tex <==
\begin{algorithm}[t!]
\caption{Negative Attention Head Probing}\label{alg:negative_attention_head_probing}
\textbf{Input: } {Probing set $X$, large language model $\psi$, number of per-sample negative attention head candidates $k$, maximum number of fine-tuned heads to be fine-tuned $N$, set of all layer and head indices $L$ and $H$, respectively.}\\
\textbf{Output: } {Fine-tuning set $D$, list of final negative attention heads $P$, early halting threshold $\tau$.} \\
\begin{algorithmic}[1]
\newcommand*{\Break}{\textbf{break}}

\State $D=S=\O$
\For{each $x_i \in X$}
    \State Let $P^i=\{(l^i_1, h^i_1), (l^i_2, h^i_2), \dots, (l^i_k, h^i_k)\}$ represent layer and head indices of top-$k$ attention heads based on single head NAS on $x_i$.
    \State $p \gets \psi(x_i)$
    \If {$p$ is positive}
        \State Append $\text{NAS}(\{x_i\}, L, H)$ to $S$
    \ElsIf {$p$ is negative}
        \State Append $x_i$ to $D$
    \EndIf
\EndFor
\State Let $P=\{(l_1, h_1), (l_2, h_2), \dots, (l_N, h_N)\}$ as the set of top-$N$ attention heads based on single head NAS on $X$ that appear in at least 90\% of $P^1, \dots, P^{|X|}$.
\State Let $\tau$ be the minimum of $S$
\State \Return $D, P, \tau$
\end{algorithmic}
\end{algorithm}

==> figures/yesno_ratio_.tex <==
\begin{figure*}[!t]
  \includegraphics[width=\textwidth]{figures/yesno_ratio.pdf}
  \caption{The ratio of ``Yes'' to ``No'' responses across different LLMs and datasets.}
  \label{fig:yesno_ratio}
\end{figure*}

==> sections/6.4_Impact_of_CoT_to_Negative_Bias.tex <==
\subsection{Impact of Chain-of-Thoughts Reasoning to Negative Bias}

==> sections/6.5_Comprehensive_Eval_with_GPT4.tex <==
\subsection{Comprehensive Evaluation with GPT-4}

==> sections/6.6_Negative_Bias_in_Foundation_Models.tex <==
\subsection{Negative Bias in Foundation Models}

==> sections/6.7_Ablation_Study.tex <==
\subsection{Ablation Study}

==> sections/B_prompts.tex <==
\section{Prompts for GPT-4} \label{B_prompts}

==> tables/neg_heads_drop.tex <==
\begin{table}[t]
    \centering
    {\resizebox{\columnwidth}{!}{
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{l|ccc}
    \toprule
      \textbf{Model}   & LLaMA 3 & Mistral & Gemma \\ \hline
       \textbf{Neg.} & - & -  & - \\
       \textbf{non-Neg}. & -  & - & - \\
     \bottomrule
    \end{tabular}
    }}    
    \caption{Average difference of NAS of each model for dropping negative or non-negative head.}
    \label{tab:neg_heads_dropping}
\end{table}

==> tables/tmp_few_shot.tex <==
\begin{table*}[t!]
\centering\caption{Results on few-shot scenario (baseline / NASA model).}
\begin{tabular}{llccc}
\toprule
\textbf{Model} & \textbf{Dataset} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\
\midrule
LLaMA & StrategyQA & \textbf{0.899} / 0.872 & 0.812 / \textbf{0.851} & 0.853 / \textbf{0.862} \\
      & GSM8K      & \textbf{0.543} / 0.532 & 0.720 / \textbf{0.870} & 0.619 / \textbf{0.661} \\
      & AR-LSAT    & 0.562 / \textbf{0.557} & 0.431 / \textbf{0.590} & 0.488 / \textbf{0.573} \\
\midrule
Mistral & StrategyQA & \textbf{0.877} / 0.832 & 0.824 / \textbf{0.889} & 0.850 / \textbf{0.859} \\
        & GSM8K      & \textbf{0.548} / 0.522 & 0.763 / \textbf{0.885} & 0.638 / \textbf{0.656} \\
        & AR-LSAT    & \textbf{0.552} / 0.532 & 0.589 / \textbf{0.720} & 0.570 / \textbf{0.612} \\
\midrule
Gemma   & StrategyQA & \textbf{0.903} / 0.897 & 0.654 / \textbf{0.659} & 0.758 / \textbf{0.760} \\
        & GSM8K      & 0.588 / \textbf{0.590} & 0.876 / \textbf{0.894} & 0.704 / \textbf{0.711} \\
        & AR-LSAT    & \textbf{0.550} / 0.535 & 0.366 / \textbf{0.405} & 0.439 / \textbf{0.461} \\
\midrule
Qwen    & StrategyQA & \textbf{0.901} / 0.894 & 0.770 / \textbf{0.805} & 0.830 / \textbf{0.847} \\
        & GSM8K      & \textbf{0.596} / 0.569 & 0.765 / \textbf{0.827} & 0.670 / \textbf{0.674} \\
        & AR-LSAT    & 0.535 / \textbf{0.546} & 0.194 / \textbf{0.303} & 0.285 / \textbf{0.390} \\
\bottomrule
\end{tabular}
\label{tab:metrics}
\end{table*}

==> tables/tmp_statistical_significance.tex <==
\begin{table}[t!]
    \centering
    \caption{General QA reasoning ability of baseline (left of ``/'') and ours (right of ``/'').}
    {\resizebox{0.9\columnwidth}{!}{
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{l|ccc}
    \toprule       
       \textbf{Model}   & \textbf{Coefficient} & \textbf{Corrected p-value} & \textbf{R-squared}\\ \hline
       \textbf{LLaMA3-8B} & $-$3.04 & $7.18\, \mathrm{E}{-01}$ & 0.271 \\
       \textbf{Mistral-7B} & 19.57 & $1.22\, \mathrm{E}{-03}$ & 0.060  \\
       \textbf{Gemma-7B} & 29.61 & $1.23\, \mathrm{E}{-21}$ & 0.377  \\
       \textbf{Qwen2-7B} & 126.03 & $4.65\, \mathrm{E}{-69}$ & 0.265 \\
     \bottomrule
    \end{tabular}
    }}    
    \label{tab:general_reasoning}
\end{table}
